The manifold rheology of fluidized granular media

Fluidized granular media have a rich rheology: measuring shear stress $\sigma$ as a function of shear rate $\dot\gamma$, they exhibit Newtonian behavior $\sigma\sim\dot\gamma$ for low densities and shear rates, develop a yield stress for intermediate shear rates and densities approaching the granular glass transition, and finally, cross over to shear-thickening Bagnold scaling, $\sigma\sim\dot\gamma^2$. This wealth of flow-behaviors makes fluidized beds a fascinating material, but also one that is challenging to encompass into a global theory, despite its relevance for optimizing industrial processes and predicting natural hazards. We provide careful measurements spanning eight orders of magnitude in shear rate, and show that all these rheological regimes can be described qualitatively and quantitatively using the granular integration through transient formalism, a theory for glassy dynamics under shear adapted to granular fluids.

==> BagnoldCoefVSphi.tex <==
\def\particlediameter{0.000069}%m
\def\particlemass{4.30017e-10}%kg
\def\yymax{4e3}
\def\yymin{4e-2}
\def\xxmax{1000}
\def\xxmin{10}
\def\deltavalue{2.0833}

\begin{loglogaxis}    [
	width=\sizex\textwidth, height=\sizey\textwidth,
	xlabel={effective shear rate $\dot{\gamma}_\text{e}$~/\si{\per\second}},
	ylabel={Bagnold coefficient $B\text{*}$},
	ylabel style={align=center, text width=0.3\textwidth}, 
	xmin=\xxmin, xmax=\xxmax,
	ymin=\yymin, ymax=\yymax,
	mark size=2.5pt,
	scaled x ticks = false,
	mark color=black,
                enlarge y limits=0.01,
                legend columns=1 , 
                legend style={
                	fill=white,
	                legend cell align=left,
	                at={(1.0,1.0)},
	                anchor=north east,
					/tikz/column 2/.style={
                		column sep=7pt,
            			},
                    }
                ]
                
\foreach \marque/\col/\phii in {
triangle/cb/0.623,
diamond/gold/0.606,
square/ce/0.555,
pentagon/ci/0.532,
o/persiangreen!40!ci/0.495}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col,
    mark=\marque,
    only marks,
	mark size=1.6pt,
	every mark/.append style={line width=0.6pt},
    ]
    table[
    x expr = \noexpand\thisrow{GammaDot}, 	
    y expr =\noexpand\thisrow{Bstar}, 
    ]
{BagnoldOriginal_Phi\phii.data};
\noexpand\addlegendentry{\phii}
	}
	\theoryplottemp
}
\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{C}};

\end{loglogaxis}



\begin{loglogaxis}    [
	width=\sizex\textwidth, height=\sizey\textwidth,
	xlabel={},
	ylabel={},
	xmin=\xxmin, xmax=\xxmax,
	ymin=\yymin, ymax=\yymax,
	yticklabels={},
	xticklabels={},
	scaled x ticks = false,
	mark color=black,
	mark size=2.5pt,
	restrict x to domain=3:3000,
	enlarge y limits=0.01,
	legend columns=2, 
	legend style={
		fill=white,
		legend cell align=left,
		at={(1.0,1.0)},
		anchor=south west,
		/tikz/column 2/.style={
		column sep=7pt,
		},
	}
]

\foreach \PF/\marque/\col/\variable in {
\PhiQzerosix/*/c1/0.6L,
\PhiQzeroseven/triangle*/c4/0.7L,
\PhiQzeroeight/diamond*/gold/0.8L,
\PhiQone/halfcircle*/c11/1L,
\PhiQonefive/square*/c21/1.5L, 
\PhiQtwo/halfsquare left*/c23/2L,
\PhiQthree/pentagon*/c28/3L2}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col,
    mark=\marque,
    only marks,
	mark size=1.5pt,
	every mark/.append style={line width=0.6pt},
    ]
    table[
    x expr = \noexpand\thisrow{gammadotUp}*((\deltavalue^2-1)/(2*\deltavalue-1)),
    y expr =\noexpand\thisrow{BagnoldCoefUp}*(\particlediameter/\particlemass), 
    ]
{BagQ\variable.data};
	}
	\theoryplottemp
}

\end{loglogaxis}


==> ShearBanding-fit-parameters.tex <==
\def\widthfigure{0.25}
\def\heightfigure{0.2}
\def\shiftiny{-15pt}
\def\shiftinx{-7pt}
\def\Di{0.024}%given in meters
\def\Do{0.050}%given in meters

\definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}

\begin{loglogaxis}    [
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	yshift=\heightfigure\textwidth+\shiftiny,
	xlabel={effective shear rate $\dot{\gamma}_\text{e}$~/\si{\per\second}},
	ylabel={shear stress $\sigma$~/\si{\pascal}},
	xmin=6e-4,
	xmax=1e3,
	ymin=9e-3,
	ymax=3e2,
	mark size=2pt,
	enlarge x limits=0.05,
	enlarge y limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	legend columns=1, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,0)},
		anchor=south east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]

\addplot [
very thick,
densely dashed,
color = c4!90,
	]
    table[
    	col sep=tab,
        x expr = ((2*(\Do/\Di)^2)/((\Do/\Di)^2-1))*2*pi*\thisrow{U}, 
        y expr = \thisrow{sigma},
]
{ExGITT/ExGITTouterfast.data};
\addlegendentry{outer}

\addplot [
very thick,
densely dashed,
color = c4!90,
forget plot
	]
    table[
    	col sep=tab,
        x expr = ((2*(\Do/\Di)^2)/((\Do/\Di)^2-1))*2*pi*\thisrow{U}, 
        y expr = \thisrow{sigma},
]
{ExGITT/ExGITTouterslow.data};

\addplot [
very thick,
solid,
color = c4!90,
	]
    table[
    	col sep=tab,
        x expr = ((2*(\Do/\Di)^2)/((\Do/\Di)^2-1))*2*pi*\thisrow{U}, 
        y expr = \thisrow{sigma},
]
{ExGITT/ExGITTinnerfast.data};
\addlegendentry{inner}

\addplot [
very thick,
solid,
color = c4!90,
forget plot,
	]
    table[
    	col sep=tab,
        x expr = ((2*(\Do/\Di)^2)/((\Do/\Di)^2-1))*2*pi*\thisrow{U}, 
        y expr = \thisrow{sigma},
]
{ExGITT/ExGITTinnerslow.data};




\foreach \PF/\marque/\col/\variable in {
\PhiQzeroseven/triangle*/c4/0.7L}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=black,
    mark=\marque,
	mark size=1.7pt,
    only marks,
    error bars/.cd, 
    	y dir=both, 
    	y explicit,
    ]
    table[
    	col sep=comma,
        x expr = \noexpand\thisrow{gammadotUp}, 
        y expr = \noexpand\thisrow{StressUp},
    ]
	{exp_data/69umsQ\variable.csv};
	}
	\theoryplottemp
}

\addplot[
    mark=o, thick,
	mark size=2.7pt,
    only marks,
color=purpleheart!90, 
]
coordinates{

(0.01,0.754619)
        };
\addplot[
    mark=o, thick,
	mark size=2.7pt,
    only marks,
color=amaranth,
]
coordinates{
(12.5,2.574386667)
        };
\addplot[
    mark=o, thick,
	mark size=2.7pt,
    only marks, 
color=darkorange,
]
coordinates{
(100,20.5416)
        };

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{A}};

\end{loglogaxis}


\begin{axis}    [
	ymode=log,
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	xlabel={radial coordinate $r/R_\mathrm{i}$},
	ylabel={local shear rate $\dot{\gamma}(r)$~/\si{\per\second}},
	xmin=1,
	ymax=1e2,
	enlarge x limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	forget plot style = {opacity = 0.6},
                enlarge y limits=0.09,
	legend columns=1, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,1)},
		anchor=north east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]


\addplot    [
	no marks,
thick,
color=darkorange,
	]
    table[
    	col sep=tab,
		x index = 0, 
		y index=1,
    ]
{ShearrateProfileQ0.7LExample.data};

\addplot    [
no marks,
thick, 
color=amaranth,
	]
    table[
    	col sep=tab,
		x index=0, 
		y index=2,
    ]
{ShearrateProfileQ0.7LExample.data};

\addplot    [
no marks,
thick,
color = purpleheart!90,
restrict x to domain=1:2.5,
	]
    table[
    	col sep=tab,
		x index=0, 
		y index=3,
    ]
{ShearrateProfileQ0.7LExample.data};

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{B}};

\end{axis}

\definecolor{richblack}{rgb}{0.0, 0.25, 0.25}
\definecolor{royalazure}{rgb}{0.0, 0.22, 0.66}
\definecolor{sacramentostategreen}{rgb}{0.0, 0.34, 0.25}

\definecolor{tyrianpurple}{rgb}{0.4, 0.01, 0.24}
\definecolor{redviolet}{rgb}{0.78, 0.08, 0.52}
\definecolor{vividburgundy}{rgb}{0.62, 0.11, 0.21}

\def\minimumx{0.005}
\def\maximumx{0.034}
\def\colone{vividburgundy}
\def\coltwo{sacramentostategreen!80}

\begin{axis}    [
	xshift=\widthfigure\textwidth+\shiftinx,
	yshift=\heightfigure\textwidth+\shiftiny,
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	xlabel={$u$~/\si{\meter\per\s}},
	ylabel={$n T_0$~/\si{\pascal} },
	xmin=\minimumx,
	xmax=\maximumx,
	ymin=0,
	ymax=0.6,
axis y line*=left,
separate axis lines,
first y axis line style={\colone},
ylabel style={\colone},
y tick style={\colone},
y tick label style={\colone},
	enlarge x limits=0.0,
	enlarge y limits=0.01,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	forget plot style = {opacity = 0.6},
                enlarge y limits=0.09,
	legend columns=2, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,1)},
		anchor=north east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]

\addplot    [
	no marks, \colone, thick, densely dashed,
	]
    table[
    	col sep=tab,
		y expr = \thisrow{nTzero}, 
		x expr = \thisrow{Q}*\Qtouconvwithcylinder,
    ]
	{GITTfitsUdata.data};

\addplot    [
	no marks, \colone, thick, 
	]
    table[
    	col sep=tab,
		y expr = \thisrow{nTi}, 
		x expr = \thisrow{Q}*\Qtouconvwithcylinder,
    ]
	{GITTfitsUdata.data};

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{C}};

\end{axis}

\begin{axis}    [
	xshift=\widthfigure\textwidth+\shiftinx,
	yshift=\heightfigure\textwidth+\shiftiny,
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	ylabel near ticks, yticklabel pos=right,
	xlabel={ },
	ylabel={$\omega_0$~/\si{\kilo\hertz}},
axis y line*=right,
separate axis lines,
second y axis line style={\coltwo},
ylabel style={\coltwo},
axis line style={\coltwo},
tick style={\coltwo},
	xmin=\minimumx,
	xmax=\maximumx,
	ymin=0,
	ymax=12,
	enlarge x limits=0,
	enlarge y limits=0.01,
	y tick label style={\coltwo},
	hide x axis,
	forget plot style = {opacity = 0.6},
                enlarge y limits=0.09,
	legend columns=1, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,1)},
		anchor=north east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]

\addlegendimage{no marks, thick, densely dashed, gray}
\addlegendentry{outer}
\addlegendimage{no marks, thick, gray}
\addlegendentry{inner}

\addplot    [
	no marks, \coltwo, thick, densely dashed,
	]
    table[
    	col sep=tab,
		y expr = \thisrow{omegao}/1e3,
		x expr = \thisrow{Q}*\Qtouconvwithcylinder,
    ]
	{GITTfitsUdata.data};

\addplot    [
	no marks, \coltwo, thick,
	]
    table[
    	col sep=tab,
		y expr = \thisrow{omegai}/1e3, 
		x expr = \thisrow{Q}*\Qtouconvwithcylinder,
    ]
	{GITTfitsUdata.data};

\end{axis}


\begin{axis}    [
	xshift=\widthfigure\textwidth+\shiftinx,
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	xlabel={$ \Updelta \varphi = \varphi_\text{g}  - \varphi $ },
	ylabel={$ \Updelta \varphi_\text{th} =  \varphi_\text{g}^\text{\textsc{mct}}  - \varphi_\text{th}  $ },
	xmin=0,
	xmax=1.5,
	ymin=0,
	ymax=7,
	mark size=2pt,
	enlarge x limits=0.05,
	enlarge y limits=0.05,
 xticklabel={$\pgfmathprintnumber{\tick}\%$},
 yticklabel={$\pgfmathprintnumber{\tick}\%$},
cycle list name=usualsuspectinner,
	forget plot style = {opacity = 0.6},
                enlarge y limits=0.09,
	legend columns=2, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,1)},
		anchor=north east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]

\foreach \phiexp/\phii/\markk/\col in {
\PhiQzerosix/0.5272/*/c1,
\PhiQzeroseven/0.522/triangle*/c4,
\PhiQzeroeight/0.517/diamond*/gold,
\PhiQone/0.514/halfcircle*/c11,
\PhiQonefive/0.503/square*/c21,
\PhiQtwo/0.493/halfsquare left*/c23,
\PhiQthree/0.478/pentagon*/c28}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!80!black,
	mark color = none,
    mark=\markk,
    only marks,
    ]
    table[
    	col sep=tab,
		x expr = (\phig- \phiexp)*100,
		y expr = (0.52796 - \phii)*100,
    ]
	{PackingFractions.data};
	}
	\theoryplottemp
}

\foreach \phiexp/\phio/\markk/\col in {
\PhiQzerosix/0.5267/o/c1,
\PhiQzeroseven/0.519/triangle/c4,
\PhiQzeroeight/0.512/diamond/gold,
\PhiQone/0.509/halfcircle/c11,
\PhiQonefive/0.495/square/c21,
\PhiQtwo/0.481/halfsquare right*/c23,
\PhiQthree/0.465/pentagon/c28}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!80!white,
	mark color = none,
    mark=\markk,
    only marks,
    ]
    table[
    	col sep=tab,
		x expr = (\phig - \phiexp)*100,
		y expr = (0.52796 - \phio)*100,
    ]
	{PackingFractions.data};
	}
	\theoryplottemp
}

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{D}};

\end{axis}

==> ShearBanding.tex <==
\def\widthfigure{0.45}
\def\heightfigure{0.3705}
\def\shiftinx{20pt}
\def\Di{0.021}%given in meters
\def\Do{0.050}%given in meters

\begin{loglogaxis}    [
	width=\widthfigure\textwidth, height=\heightfigure\textwidth,
	xshift=\shiftinx,
	ylabel={true shear rate $\dot{\gamma}$~/\si{\per\second}},
	xlabel={effective shear rate $\dot{\gamma}_\text{e}$~/\si{\per\second}},
	xmin=4e-4,
	xmax=1.2e3,
	ymin=1e-4,
	mark size=2pt,
	enlarge x limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	forget plot style = {opacity = 0.6},
                enlarge y limits=0.09,
	legend columns=3, 
	legend style={
		fill=none,
		legend cell align=left,
		at={(0.5,1)},
		anchor=north,
		/tikz/column 2/.style={column sep=7pt,},
		/tikz/column 4/.style={column sep=7pt,},
	}
]

\addlegendimage{no marks, thick, densely dashed, gray}
\addlegendentry{outer}
\addlegendimage{no marks, thick, gray}
\addlegendentry{inner}
\addlegendimage{no marks, very thick, black}
\addlegendentry{analytical}


\foreach \PF/\marque/\col/\variable in {
0.5234/o/c1/0.6L,
0.5190/triangle/c4/0.7L,
0.5155/diamond/gold/0.8L,
0.5093/halfcircle/c11/1.0L,
0.5078/square/c21/1.5L, 
0.5068/halfsquare left/c23/2.0L,
0.5073/pentagon/c28/3.0L}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col,
    no marks,
	line width=0.7pt,
    ]
    table[
    	col sep=tab,
        y expr = \noexpand\thisrow{gammadoti}, 
        x expr = \noexpand\thisrow{U}*4*pi*((\Do/\Di)^2/((\Do/\Di)^2-1)),
    ]
	{ShearRateQ/ShearRateQ\variable.data};
	}
	\theoryplottemp
}

\foreach \PF/\marque/\col/\variable in {
0.5234/o/c1/0.6L,
0.5190/triangle/c4/0.7L,
0.5155/diamond/gold/0.8L,
0.5093/halfcircle/c11/1.0L,
0.5078/square/c21/1.5L, 
0.5068/halfsquare left/c23/2.0L,
0.5073/pentagon/c28/3.0L}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!90!black,
    no marks,
    line width=0.7pt,
    dashed
    ]
    table[
    	col sep=tab,
        y expr = \noexpand\thisrow{gammadoto}, 
        x expr = \noexpand\thisrow{U}*4*pi*((\Do/\Di)^2/((\Do/\Di)^2-1)),
    ]
	{ShearRateQ/ShearRateQ\variable.data};
	}
	\theoryplottemp
}

\addplot[
	black, very thick,
	domain = 5e-4:5.2,
	samples=500, 
] {
x*(((1 - \Di/\Do)^2) / 4*pi)
};

\addplot[
	black, very thick,
	domain = 5e-4:1,
	samples=500, 
] {
(x*(((1 - \Di/\Do)^2) / 4*pi))/((\Di/\Do)^2)
};

\addplot[
	black, very thick,
	domain = 60:800,
	samples=500, 
] {
x* (sqrt(((1 - \Di/\Do)^2) / 4*(pi^2)) * (((1 - \Di/\Do)^2) / 4*pi)
};

\addplot[
	black, very thick,
	domain = 30:800,
	samples=500, 
] {
x* (sqrt(((1 - \Di/\Do)^2) / 4*(pi^2))/(\Di/\Do) * (((1 - \Di/\Do)^2) / 4*pi)
};

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{E}};
\end{loglogaxis}


==> fit-parameters.tex <==
\def\widthfigure{0.3}
\def\heightfigure{0.24}
\def\shiftiny{-15pt}
\def\shiftinx{-13pt}

\begin{axis}[
width=\widthfigure\textwidth, height=\heightfigure\textwidth,
yshift=\heightfigure\textwidth+\shiftiny,
xshift=\shiftinx,
xlabel={$\dot{\gamma} / \omega_0$},
clip mode=individual,
xmode = log,
	ymin=0.455,
	ymax=0.545,
ylabel={},
ytick={},
yticklabels ={},
	xmin=6e-9,
	xmax=2e-1,
]

\addplot graphics [
	ymin=0.45,
	ymax=0.55,
	xmin=1e-9,
	xmax=2e-1,
] {im/colormapEpsilon0.8-cut};

\coordinate (colormappos) at (rel axis cs:1,1);

\foreach \phiexp/\phio/\marque/\col/\variable  in {
\PhiQzerosix/0.5267/o/c1/0.6L,
\PhiQzeroseven/0.519/triangle/c4/0.7L,
\PhiQzeroeight/0.512/diamond/gold/0.8L,
\PhiQone/0.509/halfcircle/c11/1.0L,
\PhiQonefive/0.495/square/c21/1.5L, 
\PhiQtwo/0.481/halfsquare right*/c23/2.0L,
\PhiQthree/0.465/pentagon/c28/3.0L}{
\edef\temp{
    \noexpand\addplot [
    mark=\marque,
	mark size = 1.pt,
	color=black,
	mark color = none,
    only marks]
    table[
		x expr = \noexpand\thisrow{gammadotioveromega0},
        y expr=\noexpand\thisrow{gammadotioveromega0}/\noexpand\thisrow{gammadotioveromega0}*\phio,
    	col sep=tab,
    ]	
	{StressDimentionless/StressDimensionlessQ\variable-outer.data};
}\temp
}

\foreach \phiexp/\phii/\marque/\col/\variable  in {
\PhiQzerosix/0.5272/*/c1/0.6L,
\PhiQzeroseven/0.522/triangle*/c4/0.7L,
\PhiQzeroeight/0.517/diamond*/gold/0.8L,
\PhiQone/0.514/halfcircle*/c11/1.0L,
\PhiQonefive/0.503/square*/c21/1.5L, 
\PhiQtwo/0.493/halfsquare left*/c23/2.0L,
\PhiQthree/0.478/pentagon*/c28/3.0L}{
\edef\temp{
    \noexpand\addplot [
    mark=\marque,
	mark size = 1.pt,
	color=black,
	mark color = none,
    only marks,]
    table[
		x expr = \noexpand\thisrow{gammadotioveromega0},
        y expr=\noexpand\thisrow{gammadotioveromega0}/\noexpand\thisrow{gammadotioveromega0}*\phii,
    	col sep=tab,
    ]	
	{StressDimentionless/StressDimensionlessQ\variable-inner.data};
}\temp
}

\end{axis}

\begin{axis}[
width=\widthfigure\textwidth, height=\heightfigure\textwidth,
yshift=\heightfigure\textwidth+\shiftiny,
xshift=\shiftinx,
	color=black,
	mark color = none,
xticklabels ={},
xlabel={},
xtick={},
ytick={},
xmode = log,
	ymin=0.455,
	ymax=0.545,
ylabel={$\Updelta\varphi_\text{th} = \varphi_\text{g}^\text{MCT} - \varphi_\text{th} $},
ytick={0.46796, 0.48796, 0.50796, 0.52796},
yticklabels ={6\%, 4\%, 2\%, 0\%},
	xmin=6e-9,
	xmax=2e-1,
]
\node [anchor=north west, white] at (rel axis cs:0,1) () {\normalsize \textbf{B}};
\node [anchor=north,white ] at (rel axis cs:0.5,1) () {\small $\eta \propto \dot{\gamma}^R$};

\end{axis}

\begin{scope}[]
\def\spaceh{30.1}
\node[anchor={north east},text width=23pt, xshift=19.9pt, yshift=5.3pt] (barnumb) at ($(colormappos)+(0.5,0)$) 
{-\,1\\[\spaceh pt]-\,0\\[\spaceh pt]-\,$-1$};

\node[anchor={north west}, yshift=2.5pt] at (colormappos)  (colormap) {\includegraphics[height=76.5pt]{im/colormapEpsilon0.8-colorbar}};

\draw [] ($(colormappos)+(0.09, 0)$) rectangle ($(colormappos)+(0.29,-2.68)$);

\node[right =-18pt of barnumb] {$R$};

\end{scope}

\begin{axis}    [
width=\widthfigure\textwidth, height=\heightfigure\textwidth,
xshift=\shiftinx,
	xlabel={packing fraction $\varphi$},
	ylabel={compressibility factor $Z$},
	xmin=0.504, xmax=0.52,
	ymin=0,
	ymax=16,
	mark size=2pt,
	enlarge x limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,0)},
		anchor=south east,
	}
]

\foreach \phiexp/\phio/\Zo/\markk/\col in {
\PhiQzerosix/0.5267/11.532659192439878/*/c1,
\PhiQzeroseven/0.519/12.087009676252501/triangle*/c4,
\PhiQzeroeight/0.512/11.44950661986798/diamond*/gold,
\PhiQone/0.509/12.32458845502934/halfcircle*/c11,
\PhiQonefive/0.495/10.368523176433364/square*/c21,
\PhiQtwo/0.481/9.359605295894385/halfsquare left*/c23,
\PhiQthree/0.465/7.7678963415037/pentagon*/c28}{
    \edef\theoryplottemp{\noexpand\addplot [
	color = gray,
	fill=\col!70!white,
    mark=\markk,
    only marks,
    ]
    table[
    	col sep=tab,
		x expr = \phiexp,
		y expr = \Zo,
    ]
	{PackingFractions.data};
	}
	\theoryplottemp
}

\foreach \phiexp/\phii/\Zi/\markk/\col in {
\PhiQzerosix/0.5272/11.295080413663035/*/c1,
\PhiQzeroseven/0.522/11.809834434346186/triangle*/c4,
\PhiQzeroeight/0.517/11.089178805389777/diamond*/gold,
\PhiQone/0.514/13.10701456646773/halfcircle*/c11,
\PhiQonefive/0.503/10.471473980569993/square*/c21,
\PhiQtwo/0.493/9.327576156829657/halfsquare left*/c23,
\PhiQthree/0.478/8.075527993390232/pentagon*/c28}{
    \edef\theoryplottemp{\noexpand\addplot [
	fill=\col!90!black,
    mark=\markk,
    only marks,
    ]
    table[
    	col sep=tab,
		x expr = \phiexp,
		y expr = \Zi,
    ]
	{PackingFractions.data};
	}
	\theoryplottemp
}

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{C}};

\end{axis}


==> fitted-flowcurves.tex <==
\def\maxx{2e-1}
\def\minx{2e-9}
\def\miny{9e-4}
\def\maxy{5e4}

\def\widthofgraph{0.68}
\def\heightofgraph{0.45}

\begin{loglogaxis}    [
	width=\widthofgraph\textwidth, height=\heightofgraph\textwidth, 
	xlabel={},
	ylabel={},
	ymin=\miny, ymax=\maxy,
	xmin=\minx, xmax=\maxx,
	mark size=1.5pt,
	ytick = {1e-3,1e-2,1e-1,1e0,1e1,1e2,1e3,1e4},
	yticklabels={},
	xticklabels={},
	scaled x ticks = false,
	hide y axis,
	hide x axis,
	enlarge x limits=0,
	enlarge y limits=0,
	legend columns=1, 
	legend style={
		draw=none,
		font=\tiny,
		fill=none,
		legend cell align=left,
		at={(0.37 ,0.9)},
		anchor=north,
	}
]

\foreach \PF/\marque/\col/\variable/\Q in {
\PhiQzerosix/*/c1/0.6L/0.6,
\PhiQzeroseven/triangle*/c4/0.7L/0.7,
\PhiQzeroeight/diamond*/gold/0.8L/0.8,
\PhiQone/halfcircle*/c11/1.0L/1,
\PhiQonefive/square*/c21/1.5L/1, 
\PhiQtwo/halfsquare left*/c23/2.0L/2,
\PhiQthree/pentagon*/c28/3.0L/3}{
    \edef\theoryplottemp{\noexpand\addplot [
	color = gray,
	fill=\col!70!white,
    mark=\marque,
    only marks,
	line width=0.6pt
    ]
    table[
		x index=0, 
		y index=1,
    	col sep=tab,
    ]	
	{StressDimentionless/StressDimensionlessQ\variable-outer.data};
\noexpand\addlegendentry{\num[round-mode = places, round-precision = 3]{\fpeval{\Qtouconvwithcylinder*\Q}} }
	}
	\theoryplottemp
}

\end{loglogaxis}

\begin{loglogaxis}    [
	width=\widthofgraph\textwidth, height=\heightofgraph\textwidth, 
	xlabel={},
	ylabel={},
	ymin=\miny,
	ymax=\maxy,
	xmin=\minx,
	xmax=\maxx,
	mark size=1.5pt,
	ytick = {1e-3,1e-2,1e-1,1e0,1e1,1e2,1e3,1e4},
	yticklabels={},
	xticklabels={},
	scaled x ticks = false,
	hide y axis,
	hide x axis,
	enlarge x limits=0,
	enlarge y limits=0,
	legend columns=1, 
	legend style={
		draw=none,
		font=\tiny,
		fill=none,
		legend cell align=left,
		at={(0.218,0.9)},
		anchor=north,
	}
]

% phii
\foreach \phii/\col/\percenttogt in {
0.527/c1/0.1,
0.522/c4/0.6,
0.517/gold/1.1,
0.514/c11/1.4,
0.503/c21/2.5,
0.493/c23/3.5,
0.475/c28/5.0}{
    \edef\theoryplottemp{\noexpand\addplot [
    solid, 
	color=\col,
    no marks,
    line legend]
    table[
        x expr =\noexpand\thisrow{peclet}*sqrt(\noexpand\thisrow{T/T0}), 
        y expr =\noexpand\thisrow{sigma/nT}*\noexpand\thisrow{T/T0},
    ]
    {data_epsilon=0.80/Jc\phii-0.80.dat};
\noexpand\addlegendentry{\percenttogt\%}
	}
	\theoryplottemp
}

\end{loglogaxis}

\begin{loglogaxis}    [
	width=\widthofgraph\textwidth, height=\heightofgraph\textwidth, 
	xlabel={},
	ylabel={},
	ymin=\miny,
	ymax=\maxy,
	xmin=\minx,
	xmax=\maxx,
	mark size=1.5pt,
	ytick = {1e-3,1e-2,1e-1,1e0,1e1,1e2,1e3,1e4},
	yticklabels={},
	xticklabels={},
	scaled x ticks = false,
	hide y axis,
	hide x axis,
	enlarge x limits=0,
	enlarge y limits=0,
	legend columns=1, 
	legend style={
		draw=none,
		font=\tiny,
		fill=none,
		legend cell align=left,
		at={(0.5,0.9)},
		anchor=north,
	}
]

\foreach \phio/\col  in {
0.527/c1,
0.519/c4,
0.512/gold,
0.509/c11,
0.495/c21,
0.481/c23,
0.465/c28}{
    \edef\theoryplottemp{\noexpand\addplot [
	dashed,
	color=\col,
    forget plot,
    no marks,
    line legend]
    table[
        x expr =\noexpand \thisrow{peclet}*sqrt(\noexpand\thisrow{T/T0}), 
        y expr =\noexpand \thisrow{sigma/nT}*\noexpand\thisrow{T/T0}
    ]
    {data_epsilon=0.80/Jc\phio-0.80.dat};
	}
	\theoryplottemp
}

\addlegendimage{color=c1, no marks, dashed,}
\addlegendentry{0.1\%}
\addlegendimage{color=c4, no marks, dashed,}
\addlegendentry{0.9\%}
\addlegendimage{color=gold, no marks, dashed,}
\addlegendentry{1.6\%}
\addlegendimage{color=c11, no marks, dashed,}
\addlegendentry{1.9\%}
\addlegendimage{color=c21, no marks, dashed,}
\addlegendentry{3.3\%}
\addlegendimage{color=c23, no marks, dashed,}
\addlegendentry{4.7\%}
\addlegendimage{color=c28, no marks, dashed,}
\addlegendentry{6.3\%}

\coordinate (insetPosition) at (rel axis cs:0.923,0.1);
\end{loglogaxis}

\begin{loglogaxis}    [
	width=\widthofgraph\textwidth, height=\heightofgraph\textwidth, 
	xlabel={dimensionless shear rate $\dot{\gamma} / \omega_0$},
	ylabel={dimensionless shear stress $\sigma / nT_0$},
	ymin=\miny,
	ymax=\maxy,
	xmin=\minx,
	xmax=\maxx,
	mark size=1.5pt,
	forget plot style = {opacity = 0.6},
	%enlarge x limits=0.01,
	ytick = {1e-3,1e-2,1e-1,1e0,1e1,1e2,1e3,1e4},
	%yticklabels={},
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
	},
%	hide y axis,
%	axis x line*=bottom,
	enlarge x limits=0,
	enlarge y limits=0,
	legend columns=1, 
	legend style={
		draw=none,
		font=\tiny,
		fill=none,
		legend cell align=left,
		at={(rel axis cs: 0.095, 0.9)},
		anchor=north,
		/tikz/column 2/.style={column sep=8pt},
	}
]

\node [anchor=north west] at (rel axis cs:0, 1) () {\normalsize \textbf{A}};

\foreach \PF/\deltaPF/\marque/\col/\variable/\Q in {
\PhiQzerosix/0.1\%/*/c1/0.6L/0.6,
\PhiQzeroseven/0.6\%/triangle*/c4/0.7L/0.7,
\PhiQzeroeight/1.1\%/diamond*/gold/0.8L/0.8,
\PhiQone/1.4\%/halfcircle*/c11/1.0L/1,
\PhiQonefive/2.5\%/square*/c21/1.5L/1.5, 
\PhiQtwo/3.5\%/halfsquare left*/c23/2.0L/2,
\PhiQthree/5.0\%/pentagon*/c28/3.0L/3}{
    \edef\theoryplottemp{\noexpand\addplot [
    mark=\marque,
	fill=\col!90!black,
    only marks,
	line width=0.6pt
    ]
    table[
		x index=0, 
		y index=1,
    	col sep=tab,
    ]	
	{StressDimentionless/StressDimensionlessQ\variable-inner.data};
\noexpand\addlegendentry{\num[round-mode = places, round-precision = 3]{\fpeval{\Qtouconvwithcylinder*\Q}} }
	}
	\theoryplottemp
}

\end{loglogaxis}

\draw [] (0.4, 3.58) rectangle (5.97, 6.41);

\node[anchor=north, font=\scriptsize] at (1.6, 6.33) (inner){\quad~\,inner};
\node[below = -2.5pt of inner, font=\scriptsize](innerb)
{$u$~/\si{\meter\per\s} \hspace{5mm} $\Updelta\varphi_\text{th}$};
\node[anchor=north, font=\scriptsize] at (4.5, 6.33) (outer) {\quad~\,outer}; 
\node[below = -2.5pt of outer, font=\scriptsize]()
{$u$~/\si{\meter\per\s} \hspace{5mm} $\Updelta\varphi_\text{th}$};






==> fluidized-bed-pictures.tex <==
\def\picwidth{44}

\begin{scope}[xshift=165pt, yshift=61pt]
\node[anchor=south east] (photo1) at (0.1,-0.2) {
	\includegraphics[width=\picwidth pt, trim= 60pt 5pt 62pt 21pt, clip]{im/5Lpermin}};
\node[fill=white, opacity=0.6, anchor=south west, yshift=2pt, xshift=2pt, text opacity=1, minimum width=\picwidth pt] () at (photo1.south west) {\scriptsize$u = 0.043$\,\si{\meter\per\second}};%Q=5L/min
\node[white, anchor=north west, yshift=-2pt, xshift=1pt,] () at (photo1.north west) {\normalsize\textbf{E}};

\node[left=-3pt of photo1] (photo2) {
\includegraphics[width=\picwidth pt, trim= 60pt 5pt 62pt 21pt, clip]{im/0.8Lpermin}};
\node[rectangle, fill=white, opacity=0.6, anchor=south west, yshift=2pt, xshift=0.5pt, text opacity=1, minimum width=46pt, minimum height=10.4pt] () at (photo2.south west) {};%Q=0.8L/min
\node[anchor=south west, yshift=2pt, xshift=0.5pt, text opacity=1, minimum width=\picwidth pt] () at (photo2.south west) {\scriptsize$u = 0.0069$\,\si{\meter\per\second}};%Q=0.8L/min
\node[white, anchor=north west, yshift=-2pt, xshift=1pt,] () at (photo2.north west) {\normalsize\textbf{D}};

\node[left=-3pt of photo2] (photo3) {
\includegraphics[width=\picwidth pt, trim= 60pt 5pt 62pt 21pt, clip]{im/0Lpermin_start}};
\node[fill=white, opacity=0.6, anchor=south west, yshift=2pt, xshift=2pt, text opacity=1, minimum width=45 pt] () at (photo3.south west) {\scriptsize$u = 0$\,\si{\meter\per\second}};%Q=0L/min (start)
\node[white, anchor=north west, yshift=-2pt, xshift=1pt] (aaa) at (photo3.north west) {\normalsize\textbf{C}};

\end{scope}

==> pressure-drop.tex <==
\def\widthplots{0.284}
\def\lengthplots{0.194}
\def\xminplots{-0.002}
\def\xmaxplots{0.0485}

\begin{axis}    [
	yshift=0.11\textwidth,
	width=\widthplots\textwidth, height=\lengthplots\textwidth,
	xlabel={},
	xticklabels = {,},
	ylabel={$\mathsf{\Delta} p$},
	xmin=\xminplots, xmax=\xmaxplots,          
	ymin=0,	ymax=1.15,
	domain=0:5,
	mark size=1pt,
        ytick = {0,1},
	yticklabels={$0$, $\frac{Mg}{\pi R_o^2}$},
	enlarge x limits=0.05,	enlarge y limits=0.05,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	legend style={
		legend cell align=left,
		at={(1,0)},
		anchor=south east,
		fill=none,
	}
]

% Q minimum fluidization 
\addplot [  no marks, 
            lightgray,
            thick,
            forget plot
            ]
coordinates
{
(0.002875, -1)
(0.002875, 2)
};
\addplot [  no marks, 
            lightgray,
            thick,
            forget plot
            ]
coordinates
{
(0.010768, -1)
(0.010768, 2)
};
% MAIN PLOT
\addplot 
[   mark=diamond,
    %only marks, 
    mark size=1.5pt, 
%    mark size=3.5pt, 
	darkgray,
    %purple!80!black
    %mark options={solid, color=persianindigo}
    ]
table[
    x expr = \thisrow{Q_up_Lpermin}*\Qtouconv, 	
    y expr = \thisrow{deltap_up_Pa}/620, 
%    y error=xer1.0E5,
    col sep=comma]
{pdrop_Glass69.data};
%{images_ASdata/pdrop_Glass69.csv};
\addlegendentry{fluidization};


\addplot
[   mark=square, 
	persiangreen,
	%    purple,
    %only marks, 
%    mark size=1pt, 
    %mark options={solid, color=darkorange}
]
table[
    x expr = \thisrow{Q_down_Lpermin}*\Qtouconv, 	
    y expr = \thisrow{deltap_down_Pa}/620, 
%    y error=xer1.0E5,
    col sep=comma]
{pdrop_Glass69.data};
%{images_ASdata/pdrop_Glass69.csv};
\addlegendentry{de-fluidization};


\draw[<-, >=latex, gray] (axis cs: 0.002875, 0.62) -- (axis cs: 0.018, 0.62) node[anchor=west]{ $u_{2}\approx\SI{0.3}{\centi\metre\per\s}$};

%\node[anchor=west, gray] at (axis cs: 0.013, 0.7) () {$u_{2}$}; %=1.08 \cdot10^{-2}~\si{\meter\per\second} 
\draw[<-, >=latex, gray] (axis cs: 0.010768, 0.8) -- (axis cs: 0.018, 0.8) node[anchor=west]{ $u_{1}\approx\SI{1}{\centi\metre\per\s}$};

%\node[anchor=east] at (axis cs: 4.1, 520) () {$\frac{m \, g}{A}=\SI{624.5}{\pascal}$}; %624.5239967
%\draw[<-, >=latex] (axis cs: 4.7, 602) |- (axis cs: 4.1, 520);


\draw[<-, persiangreen] (axis cs: 0.028, 0.89) -- (axis cs: 0.037, 0.89);
\draw[->, darkgray] (axis cs: 0.028, 1.11) -- (axis cs: 0.037, 1.11);


\coordinate (insetPosition) at (rel axis cs:0.986,0.23);

\node [anchor=north west] at (rel axis cs:0, 1) () {\normalsize \textbf{A}};

\end{axis}


\begin{axis}    [
	width=\widthplots\textwidth, height=\lengthplots\textwidth,
	xlabel={gas flow velocity $u$~/\si{\m\per\s}},
	ylabel={packing fractions $\varphi$},
	ymin=0.455,
	ymax=0.688,
	xmin=\xminplots, xmax=\xmaxplots,          
	mark size=1.5pt,
	%enlarge x limits=0.01,
	%yticklabels={},
%	ytick={0.5,0.55,0.6,0.65},
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
%	hide y axis,
%	axis x line*=bottom,
	enlarge x limits=0.05,	enlarge y limits=0.05,
%	legend columns=2, 
	legend style={
	fill=none,
%	font = \footnotesize,
	legend cell align=left,
	at={(1,1)},
	anchor=north east,
	/tikz/column 2/.style={
		column sep=10pt,
		},
	}
]

%\addplot [
%	forget plot,
%	solid,
%	no marks,
%	gray, dotted, thick,
%	%y domain = 1.33e-13:1.68e-13,
%	%restrict y to domain = 1.33e-13:1.68e-13,
%	]
%	coordinates{
%	(0.0081,0.4)
%	(0.0081, 0.7)
%	};
	
%\node[anchor=west] at (axis cs: 0.011, 0.47) () {$u_{c}= 8.1 \cdot 10^{-3}~\si{\meter\per\second} $}; 
%\draw[<-, >=latex] (axis cs: 0.0081, 0.47) -- (axis cs: 0.011, 0.47);

	
	
\addplot [
	mark=triangle,
 	only marks, 
	mark size=2pt, 
	persianindigo,
    error bars/.cd, y fixed, y dir=both, y explicit] 
table[
    x expr = \thisrow{Q_Lpermin}*\Qtouconv, 	
    y=Phi, 
    y error=error_Phi,
    ]
{QvsPhiRCP.data};
\addlegendentry{\hspace{2pt} before fluidization}; %$\varphi_{\text{exp}}$ 

\addplot [  no marks, 
            lightgray,
            thick,
            forget plot
            ]
coordinates
{
(0.002875, -1)
(0.002875, 2)
};
\addplot [  no marks, 
            lightgray,
            thick,
            forget plot
            ]
coordinates
{
(0.010768, -1)
(0.010768, 2)
};

\addplot
[  		
	forget plot,
    lightgray,
    densely dashed, thick,
    no marks, 
    domain=0.004:0.0619,
    %mark size=1.5pt, 
    %mark options={solid, color=darkorange}
]
{\phiRLP+((\phiINF-\phiRLP)/(1+(\uzero /(x - \ufp))^\exposant))};
%\addlegendentry{\hspace{2pt} Fit to fluidized data};

\addplot
[   mark=o, 
    persianindigo,
    only marks, 
	mark size=2pt, 
    %mark options={solid, color=darkorange}
    error bars/.cd, y fixed, y dir=both, y explicit
]
table[
    x expr =\thisrow{Q_Lpermin}*\Qtouconv,
    y=Phi, 
    y error=error_Phi,
    ]
{QvsPhi.data};
\addlegendentry{\hspace{2pt} with fluidization}; %$\varphi_{\text{exp}}$ 

\addplot    [
	c1, mark = *,
	only marks,
	]
coordinates{
(0.6*\Qtouconvwithcylinder, \PhiQzerosix)
        };
        
\addplot    [
	c4, mark = triangle*,
	only marks,
	]
coordinates{
(0.7*\Qtouconvwithcylinder, \PhiQzeroseven)
        };
     
\addplot    [
	gold, mark = diamond*,
	only marks,
	]
coordinates{
(0.8*\Qtouconvwithcylinder, \PhiQzeroeight) 
        };
        
\addplot    [
	c11, mark = halfcircle*,
	only marks,
	]
coordinates{
(1*\Qtouconvwithcylinder, \PhiQone)
        };
        
\addplot    [
	c21, mark = square*,
	only marks,
	]
coordinates{
(1.5*\Qtouconvwithcylinder, \PhiQonefive)
        };
        
\addplot    [
	c23, mark = halfsquare right*,
	only marks,
	]
coordinates{
(2*\Qtouconvwithcylinder, \PhiQtwo)
        };
        
\addplot    [
	c28, mark = pentagon*,
	only marks,
	]
coordinates{
(3*\Qtouconvwithcylinder, \PhiQthree) 
        };


%\def\endofarrow{0.007}
%\draw[<-, >=latex] (axis cs: 0.001, 0.567144563) to (axis cs: \endofarrow, 0.567144563);
%\node [anchor=west]at (axis cs: \endofarrow, 0.567144563) (philexp) {$\varphi_{\text{exp}}^l$};
%\node [right=-2pt of philexp, anchor=west] (philexpnbr) {$= 0.567$};
%\node [below=1pt of philexpnbr.south west, anchor=north west] () {$\approx \varphi_{\text{rlp}}$};


%\draw[<-, >=latex] (axis cs: 0.001,0.636619772) to (axis cs: \endofarrow, 0.636619772);
%\node [anchor=west]at (axis cs: \endofarrow, 0.636619772) (phidexp) {$\varphi_{\text{exp}}^d$};
%\node [right=-2pt of phidexp, anchor=west] (phidexpnbr) {$= 0.637$};
%\node [below=1pt of phidexpnbr.south west, anchor=north west] () {$\approx \varphi_{\text{rcp}}$};

%\node [anchor=west]at (axis cs: 0.0088, 0.616619772) () {$\approx \varphi_{\text{rcp}}$};

\draw[<-, gray] (axis cs: 0.032, 0.487) -- (axis cs: 0.039, 0.487);

\node [anchor=north west] at (rel axis cs:0, 1) () {\normalsize \textbf{B}};

\end{axis}


==> rheometer-schematic.tex <==
%\vspace{-100pt}
\begin{scope}[scale=0.6, yshift=-20pt]
\begin{scope}[scale=0.55, yshift=18, xshift=100]
% CAMERA
\fill [gray, lightgray!20, line join = round] (0.1,0.2) rectangle (1,2);
\fill [gray, lightgray!55, line join = round] (0.1,2) -- (0.6, 2.7)-- (1.5,2.7)--(1,2);
\fill [gray, lightgray!90, line join = round] (1,2) -- (1.5, 2.7)-- (1.5,0.9)--(1,0.2);

\draw [gray, thick, line join = round] (0.1,0.2) rectangle (1,2);
\draw [gray, thick, line join = round] (0.1,2) -- (0.6, 2.7)-- (1.5,2.7)--(1,2);
\draw [gray, thick, line join = round] (1,2) -- (1.5, 2.7)-- (1.5,0.9)--(1,0.2);

\fill [lightgray!20] (1.3,1.47) ellipse (5pt and 12.2pt);
\draw[gray, thick] (1.3,1.47) ellipse (5pt and 12.2pt);
\fill [lightgray!20] (1.3, 1.04) -- (1.8, 1.04)-- (1.8,1.9)--(1.3,1.9);
\draw [gray, thick] (1.3, 1.04) -- (1.8, 1.04)-- (1.8,1.9)--(1.3,1.9);
% end of objective of camera 
\fill[white] (1.8,1.47) ellipse (5pt and 12.2pt);
\draw[gray, thick] (1.8,1.47) ellipse (5pt and 12.2pt);

\node[align=center] (camera) at (0.95, 4.5) {camera};
\node[align=center, anchor=north] (cameralegend) at (camera.south) {($\varphi$)};

\node[anchor=north west, above = 0.69 of cameralegend.west, xshift=2pt] () {\normalsize\textbf{F}};

\end{scope}



% RHEOMETER
%\fill [lightgray!55, line join = round] (3.6,6) -- (4.2,6.5)-- (7.65,6.5) -- (7.3,6);
%\fill [lightgray!90, line join = round]  (7.65,6.5) -- (7.3,6) -- (7.3,0.8) -- (7.65,1.6)--cycle;
%\fill [lightgray!10, line join = round] (3.6, 0.8) rectangle (7.3,6);
%
%\draw [gray, thick, line join = round] (3.6,6) -- (4.2,6.5)-- (7.65,6.5) -- (7.3,6);
%\draw [gray, thick, line join = round]  (7.65,6.5) -- (7.3,6) -- (7.3,0.8) -- (7.65,1.6)--cycle;
%\draw [gray, thick, line join = round] (3.6,0.8) rectangle (7.3,6);	
%
\fill [lightgray!30] (4.035,2.7) rectangle (6.565,0.3);

\fill [lightgray] (4.035,1.9) rectangle (6.565,0.2);

% glass container 1/3
\draw [thick,  lightgray!90] (4.035,2.7) rectangle (6.565,0);
\fill[darkgray] (5.3,0) ellipse (36pt and 5pt);
% glass container 2/3
\draw [thick,  lightgray!90] (5.3,0) ellipse (36pt and 5pt);
\fill [darkgray] (4.052,0) rectangle (6.547,0.2);	

\fill[thick, lightgray!15] (5.3,2.7) ellipse (36pt and 5pt);
\fill [gray] (5.25,3.2) rectangle (5.35,1);	
% glass container 3/3
\draw[thick, lightgray!90] (5.3,2.7) ellipse (36pt and 5pt);
\fill [gray] (5.25,3.2) rectangle (5.35,2.8);	

%\draw[-Stealth,black] (5,3.5) arc (200:300:0.4);
\draw[-Stealth,black, scale=1]  (5.54,2.8) arc (-50:289:0.36 and 0.13);
\fill [gray] (5.25,2.9) rectangle (5.35,3.2);	

\fill [gray, line join = round, rounded corners=0.2pt] (5.25, 3.1)--(5.25, 3.22)--(5.28, 3.24)--(5.32, 3.2)--(5.35,3.22)--(5.35, 3.1)--cycle;

% top part coming out of rheometer
%\fill [lightgray!20, line join = round] (4.034,4) rectangle (6.566,5.5);	
%\fill [lightgray!55, line join = round]  (6.566,5.5) -- (6.7,5.7)-- (4.2,5.7) -- (4.034,5.5)--cycle;
%\fill [lightgray!90, line join = round] (6.566,5.5) -- (6.7,5.7)-- (6.7,4.35) -- (6.566,4)--cycle;

%\draw [thick,gray,line join = round] (4.034,4) rectangle (6.566,5.5);	
%\draw [thick,gray,line join = round]  (6.566,5.5) -- (6.7,5.7)-- (4.2,5.7) -- (4.034,5.5)--cycle;
%\draw [thick,gray,line join = round] (6.566,5.5) -- (6.7,5.7)-- (6.7,4.35) -- (6.566,4)--cycle;

\fill[gray] (5.3,1.6) ellipse (15pt and 4pt);
\fill [gray] (4.773,0.8) rectangle (5.827,2);	
\fill[gray] (5.3,0.8) ellipse (15pt and 2pt);

%%%% FILTER %%%%
\draw [thick, black] (4.075,1.9) rectangle (6.525,0.21);
\fill[darkgray!90] (5.3,0.2) ellipse (35.5pt and 5pt);

\fill[lightgray] (5.3,1.91) ellipse (35.2pt and 5pt);
\draw[black, thick] (5.3,1.91) ellipse (35.05pt and 5pt);
\fill [gray] (5.827,2)--(5.3,2.4)--(4.773,2)--(4.773,1.9)--(5.827,1.9)--cycle;
\fill[gray] (5.3,1.9) ellipse (15pt and 2pt);

\draw[black, {Circle[open]}-] (5.42, -0.21)--(3.7, -0.21) node [anchor=east] {pressure $p$};
%node [anchor=north east, yshift=1pt] {sensor ($p$)};

\draw[black, ->, thick] (4.22,0.2)--(4.22,0.62);
\draw[black, ->, thick] (4.76,0.2)--(4.76,0.62);
\draw[black, ->, thick] (5.3,0.2)--(5.3,0.62);
\draw[black, ->, thick] (5.84,0.2)--(5.84,0.62);
\draw[black, ->, thick] (6.38,0.2)--(6.38,0.62);


\draw[black, {Circle[open]}-] (6.45, 2.2)--(7.3, 2.2) node [anchor=west] {$R_o = $~\SI{25}{\mm}};
\draw[black, {Circle[open]}-] (5.71, 1.6)--(7.3, 1.6) node [anchor=west] {$R_i = $~\SI{10.5}{\mm}};
\draw[black, {Circle[open]}-] (6.1,1.)--(7.3, 1.) node [anchor=west] {fluidized bed}; % text width=30mm granular\\ 

\draw[darkgray, thick] (6.546,0.1)--(7.3, 0.1) node [midway, above] {$u$} node [anchor=west, text width=12mm, text centered, draw, rectangle] {mass flow controller};

\node[] () at (5.3,3.5) {Anton Paar MCR-302};

%\node[anchor=north west,] () at (0,7) {\textbf{(d)}};

\end{scope}

==> stress_flowcurves.tex <==
\begin{loglogaxis}    [
	width=0.45\textwidth, height=0.304\textwidth,
	xlabel={effective shear rate $\dot{\gamma}_\text{e}$~/\si{\per\second}},
	ylabel={shear stress $\sigma$~/\si{\pascal}},
	ymin=7e-4,
	ymax=2e3,
	xmin=9e-5,
	xmax=2e3,
	mark size=1.5pt,
	forget plot style = {opacity = 0.6},
	%enlarge x limits=0.01,
	ytick = {1e-3,1e-2,1e-1,1e0,1e1,1e2,1e3},
	%yticklabels={},
	scaled x ticks = false,
%	mark color=black,
	x tick label style={
		/pgf/number format/precision=4
	},
%	hide y axis,
%	axis x line*=bottom,
	enlarge x limits=0,
	enlarge y limits=0,
	legend columns=4, 
	legend style={
%		font=\tiny,
		fill=none,
		legend cell align=left,
		at={(0.455,1)},
		anchor=north,
		/tikz/column 2/.style={column sep=5pt},
		/tikz/column 4/.style={column sep=5pt},
		/tikz/column 6/.style={column sep=5pt},
	}
]

%\addplot [  no marks, 
%            lightgray,
%            forget plot
%            ]
%coordinates
%{
%(25, 1e-4)
%(25, 1e3)
%};
\addplot [  no marks, 
            c1,
            densely dotted, thick,
            forget plot,
            ]
coordinates
{
(1e-4, 5)
(25, 5)
};

\node [anchor=south west] at (1.5e-4, 5) () {$\sigma_0 \approx$~\SI{5}{\pascal}};


\addplot [  no marks, 
            darkgray,
            forget plot, thick,
            domain=6e1:1e3
            ]
{x*1.825e-5};
%\node [above] at (1e0, 0.3926023) () {\textcolor{gray}{ $\eta = \SI{0.3926023}{\pascal\s}$ }};

\foreach \PF/\marque/\col/\variable in {
\PhiQzerosix/o/c1/0.6L,
\PhiQzeroseven/triangle/c4/0.7L,
\PhiQzeroeight/diamond/gold/0.8L,
\PhiQone/halfcircle/c11/1L,
\PhiQonefive/square/c21/1.5L, 
\PhiQtwo/halfsquare right*/c23/2L,
\PhiQthree/pentagon/c28/3L2}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!80!white,
    mark=\marque,
    forget plot,
    only marks,
	every mark/.append style={line width=0.5pt},
    error bars/.cd, 
    	y dir=both, 
    	y explicit,
    ]
    table[
    	col sep=comma,
        x expr = \noexpand\thisrow{gammadotDown}, 
        y expr = \noexpand\thisrow{StressDown},
        y error plus expr=\noexpand\thisrow{stdStressDown},
        y error minus expr=\noexpand\thisrow{stdStressDown}
    ]
	{exp_data/69umsQ\variable.csv};
%\noexpand\addlegendentry{ $\varphi_{\text{exp}}=$~\PF}
\noexpand\addlegendentry{~\PF}
	}
	\theoryplottemp
}

\foreach \PF/\marque/\col/\variable in {
\PhiQzerosix/*/c1/0.6L,
\PhiQzeroseven/triangle*/c4/0.7L,
\PhiQzeroeight/diamond*/gold/0.8L,
\PhiQone/halfcircle*/c11/1L,
\PhiQonefive/square*/c21/1.5L, 
\PhiQtwo/halfsquare left*/c23/2L,
\PhiQthree/pentagon*/c28/3L2}{
    \edef\theoryplottemp{\noexpand\addplot [
    color=\col!80!black,
    mark=\marque,
    only marks,
    error bars/.cd, 
    	y dir=both, 
    	y explicit,
    ]
    table[
    	col sep=comma,
        x expr = \noexpand\thisrow{gammadotUp}, 
        y expr = \noexpand\thisrow{StressUp},
        y error plus expr=\noexpand\thisrow{stdStressUp},
        y error minus expr=\noexpand\thisrow{stdStressUp}
    ]
	{exp_data/69umsQ\variable.csv};
%\noexpand\addlegendentry{ $\varphi_{\text{exp}}=$~\PF}
	}
	\theoryplottemp
}

%%%%%%%%%%%%%%%%%%% TRIANGLES %%%%%%%%%%%%%%%%%%%%%%
%upper triangle:
\draw [lightgray,thick] 
(axis cs:7e2,2e0)
-- (axis cs:2e2,2e0) 
-- (axis cs:7e2,3e1)
-- cycle;
\node at (axis cs:4e2, 1.7e0) [lightgray, below] {\footnotesize 1};
\node at (axis cs: 7.2e2,8.5e0) [lightgray, right] {\footnotesize 2};
%% lower triangle:
\draw [lightgray, thick] 
(axis cs:2e0, 8e-2)
-- (axis cs:2e0, 2e-3) node [midway, lightgray, right] {\footnotesize 1}
-- (axis cs:5e-2, 2e-3) node [midway, lightgray, xshift=5pt, above] {\footnotesize 1}
-- cycle;
%\node at (axis cs: 1e-1,2e-3) [lightgray, right] {\footnotesize 1};
%\node at (axis cs: 2e-2,1.1e-4) [lightgray] {\footnotesize 1};


\node [gray, anchor=south east, text width=1cm] at (rel axis cs:0.85, 0.05) () {viscosity\\of air $\eta_\text{f}$};

\node [anchor=north west] at (rel axis cs:0, 1) () {\normalsize \textbf{G}};

\end{loglogaxis}

==> viscosity-flowcurve.tex <==
\def\minimumx{2e-4}
\def\maximumx{2e3}
\def\minimumy{4e-2}
\def\maximumy{5e4}

\begin{loglogaxis}    [
	width=0.65\textwidth, height=0.45\textwidth,
	xlabel={effective shear rate $\dot{\gamma}_e$~/\si{\per\second}},
	ylabel={effective viscosity $\eta_\text{e} $~/\si{\pascal\second}},
	xmin=\minimumx,
	xmax=\maximumx,
	ymin=\minimumy,
	ymax=\maximumy,
	mark size=2pt,
	enlarge x limits=0,
	enlarge y limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	forget plot style = {opacity = 0.6},
	legend columns=7, 
	legend style={
		fill=white,
		legend cell align=left,
		at={(0.5,0.975)},
		anchor=north,
/tikz/column 2/.style={column sep=7pt,},
/tikz/column 4/.style={column sep=7pt,},
/tikz/column 6/.style={column sep=7pt,},
/tikz/column 8/.style={column sep=7pt,},
/tikz/column 10/.style={column sep=7pt,},
/tikz/column 12/.style={column sep=7pt,},
	}
]

\definecolor{backgroundyellow}{rgb}{0.99, 0.99, 0.59}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}
\definecolor{trueblue}{rgb}{0.0, 0.45, 0.81}

\addplot[name path=NewtReg, forget plot, 
draw=none,
fill=backgroundyellow, fill opacity=0.24]
coordinates
{
(\minimumx, \minimumy)
(\minimumx, 1e4)
(35, \minimumy)
};

\addplot[name path=BagReg,  forget plot, 
draw=none,
shade, left color=purple, right color=white,
fill opacity=0.22]
coordinates
{
(35, \maximumy)
(35, \minimumy)
(\maximumx, \minimumy)
(\maximumx, \maximumy)
};

\addplot [  no marks, 
			densely dashed, thick,
            c4,
            forget plot
            ]
coordinates
{
(\minimumx, 73.0863549)
(10, 73.0863549)
};

\addplot [  no marks, 
            gold,
            forget plot, densely dashed, thick,
            ]
coordinates
{
(\minimumx, 10.22648799)
(0.1, 10.22648799)
};

\addplot [  no marks, 
            c11,
            forget plot, densely dashed, thick,
            ]
coordinates
{
(\minimumx, 5.618818)
(10, 5.618818)
};

\addplot [  no marks, 
            c21,
            forget plot,densely dashed, thick,
            ]
coordinates
{
(\minimumx, 2.132328249)
(10, 2.132328249)
};

\addplot [  no marks, 
            c23,
            forget plot, densely dashed, thick,
            ]
coordinates
{
(\minimumx, 1.554748531)
(10, 1.554748531)
};

\addplot [  no marks, 
            c28,
            forget plot, densely dashed, thick,
            ]
coordinates
{
(\minimumx, 0.553189374)
(10, 0.553189374)
};

\addplot[name path=ShThinReg, forget plot,
draw=none,
fill opacity=1,
fill=trueblue!14!white]
coordinates
{
(\minimumx, 1e4)
(35, \minimumy)
(35, \maximumy)
(\minimumx, \maximumy)
};

\foreach \PF/\marque/\col/\variable in {
\PhiQzerosix/o/c1/0.6L,
\PhiQzeroseven/triangle/c4/0.7L,
\PhiQzeroeight/diamond/gold/0.8L,
\PhiQone/halfcircle/c11/1L,
\PhiQonefive/square/c21/1.5L, 
\PhiQtwo/halfsquare right*/c23/2L,
\PhiQthree/pentagon/c28/3L2}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!80!white,
    mark=\marque,
    forget plot,
    only marks,
	every mark/.append style={line width=0.6pt},
    error bars/.cd, 
    	y dir=both, 
    	y explicit,
    ]
    table[
    	col sep=comma,
        x expr = \noexpand\thisrow{gammadotDown}, 
        y expr = \noexpand\thisrow{StressDown}/\noexpand\thisrow{gammadotDown},
        y error plus expr=\noexpand\thisrow{stdStressDown}/\noexpand\thisrow{gammadotDown},
        y error minus expr=\noexpand\thisrow{stdStressDown}/\noexpand\thisrow{gammadotDown}
    ]
{exp_data/69umsQ\variable.csv};
	}
	\theoryplottemp
}

\foreach \PF/\marque/\col/\variable in {
\PhiQzerosix/*/c1/0.6L,
\PhiQzeroseven/triangle*/c4/0.7L,
\PhiQzeroeight/diamond*/gold/0.8L,
\PhiQone/halfcircle*/c11/1L,
\PhiQonefive/square*/c21/1.5L, 
\PhiQtwo/halfsquare left*/c23/2L,
\PhiQthree/pentagon*/c28/3L2}{
    \edef\theoryplottemp{\noexpand\addplot [
	color=\col!80!black,
	mark color = none,
    mark=\marque,
    only marks,
	every mark/.append style={line width=0.6pt},
    error bars/.cd, 
    	y dir=both, 
    	y explicit,
    ]
    table[
    	col sep=comma,
        x expr = \noexpand\thisrow{gammadotUp}, 
        y expr = \noexpand\thisrow{StressUp}/\noexpand\thisrow{gammadotUp},
        y error plus expr=\noexpand\thisrow{stdStressUp}/\noexpand\thisrow{gammadotUp},
        y error minus expr=\noexpand\thisrow{stdStressUp}/\noexpand\thisrow{gammadotUp}
    ]
{exp_data/69umsQ\variable.csv};
\noexpand\addlegendentry{\PF}
	}
	\theoryplottemp
}

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{A}};

\coordinate (insetPosition) at (rel axis cs:0.9,0.815);
\end{loglogaxis}

\begin{loglogaxis}    [
	font = \footnotesize,
	width=0.65\textwidth, height=0.45\textwidth,
	xlabel={},
	ylabel={},
	xmin=\minimumx,
	xmax=\maximumx,
	ymin=\minimumy,
	ymax=\maximumy,
	mark size=2pt,
	enlarge x limits=0,
	enlarge y limits=0,
	xticklabels ={},
	yticklabels ={},
	xlabel={},
	ylabel={},
	xtick={},
	ytick={},
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
		},
	forget plot style = {opacity = 0.6}
]

\end{loglogaxis}

\begin{axis}[
	font = \footnotesize,
at={(insetPosition)},anchor={north east},
width=0.28\textwidth, height=0.22\textwidth, 
xlabel={shear rate $\dot{\gamma}$},
ylabel={packing fraction $\varphi$},
xtick={1e-7, 1e-5, 1e-3,1e-1},
xticklabels ={},
yticklabels ={},
xmode = log,
	ymin=0.5,
	ymax=0.53,
	xmin=7e-9,
	xmax=2e-1,
]
\addplot graphics [
	ymin=0.5,
	ymax=0.53,
	xmin=7e-9,
	xmax=2e-1,
] {im/colormapEpsilon0.8-cut};
\coordinate (colormappos) at (rel axis cs:1,1);

\end{axis}

\begin{axis}[
	font = \footnotesize,
at={(insetPosition)}, anchor={north east}, footnotesize,
width=0.28\textwidth, height=0.22\textwidth, 
title ={$\eta \propto \dot{\gamma}^R$},
xticklabels ={},
yticklabels ={},
xlabel={},
ylabel={},
xtick={},
ytick={},
xmode = log,
	ymin=0.5,
	ymax=0.53,
	xmin=7e-9,
	xmax=2e-1,
]

\end{axis}

\node[anchor={north west}, yshift=2.7pt] at (colormappos)  (colormap) {\includegraphics[height=66.7pt]{im/colormapEpsilon0.8-colorbar}};

\draw [] ($(colormappos)+(0.08,0)$) rectangle ($(colormappos)+(0.26,-2.33)$);

\def\spaceh{25.1}
\node[anchor={north east},text width=18pt, xshift=21.8pt, yshift=5.6pt] (barnumb) at ($(colormappos)+(0.25,-0.01)$) 
{-\,1\\[\spaceh pt]-\,0\\[\spaceh pt]-\,$-1$};
\node[right =-12pt of barnumb] {$R$};



==> viscosityVSphi.tex <==
\begin{axis}    [
	ymode=log,
	yshift=\shiftiny\textwidth,
	width=\sizex\textwidth, height=\sizey\textwidth,
	xlabel={packing fraction $\varphi $},
	ylabel={Newtonian viscosity $ \eta_\text{N}$~/\si{\pascal\second}},
	xmin=0.505, xmax=0.52,
	ymin=6e-2, ymax=1e6,
	mark size=2.5pt,
	enlarge x limits=0,
	enlarge y limits=0,
	scaled x ticks = false,
	x tick label style={
		/pgf/number format/precision=4
	},
	legend style={
		fill=none,
		legend cell align=left,
		at={(1,1)},
		anchor=north east,
		/tikz/column 2/.style={
			column sep=7pt,
		},
	}
]

\def\ymin{\pgfkeysvalueof{/pgfplots/ymin}}
\def\ymax{\pgfkeysvalueof{/pgfplots/ymax}}

\addplot    [
	dashed, gray, 
	no marks,
]
coordinates{
(\phig, \ymin)
(\phig, \ymax)
        };

\node [anchor=south east, gray] at (\phig, 1e-1) {$\varphi_\text{g} = \phig$};

\addplot[
	gray,
	domain = 0.505:0.519,
	samples=500, 
] {
(\etazero)/((\phig-x)^(\etaequation))
};

\addplot    [
	c1!80!black, mark = *,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQzerosix, 4154.61501) +- (923.1488389, 923.1488389)
        };

\addplot    [
	c4!80!black, mark = triangle*,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQzeroseven, 73.0863549) +- (13.73322466,13.73322466)
        };
     
\addplot    [
	gold!80!black, mark = diamond*,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQzeroeight, 10.22648799) +- (1.921882613, 1.921882613)
        };
        
\addplot    [
	mark = halfcircle*,
	color=c11!80!black,
	mark color = none,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQone, 5.618818) +- (0.606435363, 0.606435363)
        };
        
\addplot    [
	c21!80!black, mark = square*,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQonefive, 2.132328249) +- (0.671738552, 0.671738552)
        };
        
\addplot    [
	mark = halfsquare left*,
	color=c23!80!black,
	mark color = none,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQtwo, 1.554748531) +- (0.993474566, 0.993474566)
        };
        
\addplot    [
	c28!80!black, mark = pentagon*,
	only marks,
	    error bars/.cd, 
    	y dir=both, 
    	y explicit,
	]
coordinates{
(\PhiQthree, 0.553189374) +- (0.785477958, 0.785477958)
        };

\node [anchor=north west] at (rel axis cs:0,1) () {\normalsize \textbf{B}};

\end{axis}
